Harness-Driven Agentic Operation of Optical Pooled Screen Analysis

Optical pooled screens connect genetic perturbations to changes in cell morphology and behavior, but turning the microscopy data into interpretable results takes complex, multi-day analyses. Established pipelines process this data, yet researchers still select parameters, inspect outputs, and resolve failures for each experiment. Here, we present Brieflow-auto, a pipeline-specific harness implemented as a Claude Code plugin that lets a coding large language model (LLM) operate Brieflow, an open-source end-to-end pipeline for optical pooled screening data. A researcher supplies experimental facts and approves the launch. An agent tunes parameters in an interactive notebook, and the harness validates the configuration, monitors execution, recovers from common failures, and checks output quality. For pipeline defects, the agent opens upstream issues proposing backward-compatible fixes for the broader community. In five previously analyzed screens, harness runs yielded more cells with a confident single-gene assignment than the original hand analyses. On a screen the pipeline was not designed for, the harness turned each failure into a reviewed upstream fix. More broadly, we propose that wrapping an established pipeline in a harness can substantially accelerate its use and the long-term reliability of its codebase.

==> figures/schematic_style.tex <==
\usepgflibrary{arrows.meta}%

\providecommand{\schHead}{\sffamily\fontsize{8.6}{9.8}\selectfont}%
\providecommand{\schBody}{\sffamily\fontsize{7.6}{8.8}\selectfont}%
\providecommand{\schSmall}{\sffamily\fontsize{7.1}{8.2}\selectfont}%
\providecommand{\schTiny}{\sffamily\fontsize{6.8}{7.8}\selectfont}%
\providecommand{\schNum}{\sffamily\fontsize{10.5}{11.6}\selectfont\bfseries}%
\providecommand{\schMono}{\ttfamily\fontsize{6.8}{7.8}\selectfont}%

\colorlet{schAgentFill}{blue!10}
\colorlet{schAgentLine}{blue!48}
\colorlet{schHumanFill}{orange!15}
\colorlet{schHumanLine}{orange!65}
\colorlet{schRecordFill}{black!6}
\colorlet{schRecordLine}{black!32}
\colorlet{schLine}{black!45}
\colorlet{schArrow}{black!55}
\colorlet{schArrowBold}{black!72}
\colorlet{schText}{black!82}
\colorlet{schMuted}{black!55}
\colorlet{schBandFill}{black!3}
\colorlet{schBandLine}{black!16}

\tikzset{
  schbox/.style={draw=schLine,line width=0.55pt,rounded corners=2.4pt,align=center,
    font=\schBody,inner sep=4pt,fill=white},
  schagent/.style={schbox,fill=schAgentFill,draw=schAgentLine},
  schhuman/.style={schbox,fill=schHumanFill,draw=schHumanLine},
  schrecord/.style={schbox,fill=schRecordFill,draw=schRecordLine},
  schchip/.style={schbox,font=\schSmall,inner sep=3pt,minimum height=0.46cm},
  schband/.style={rounded corners=3.5pt,line width=0.5pt,draw=schBandLine,fill=schBandFill},
  schbandmain/.style={rounded corners=3.5pt,line width=0.8pt,draw=schAgentLine!70,
    fill=blue!4},
  schsleeve/.style={rounded corners=4pt,line width=0.8pt,draw=schAgentLine,
    dash pattern=on 2.0pt off 1.5pt},
  schflow/.style={-{Latex[length=2.0mm,width=1.45mm]},line width=0.6pt,draw=schArrow},
  schloop/.style={-{Latex[length=2.6mm,width=1.85mm]},line width=1.05pt,
    draw=schArrowBold,rounded corners=3pt},
  schlink/.style={line width=0.45pt,draw=schLine},
  schnote/.style={font=\schTiny,text=schMuted,align=center,inner sep=1pt},
  schlabel/.style={font=\schBody,text=black!78,align=center,inner sep=2pt},
  schhead/.style={font=\schHead,anchor=north west,inner sep=0pt,text=schText},
  schbadge/.style={rounded corners=1.6pt,fill=schHumanFill,draw=schHumanLine,
    line width=0.35pt,inner sep=0pt,minimum width=0.80cm,minimum height=0.30cm,
    font=\schTiny,text=black!65},
  schstrip/.style={rounded corners=2.5pt,line width=0pt,draw=none,fill=schBandFill},
  schstep/.style={schbox,minimum height=0.46cm,inner sep=3pt},
  schring/.style={schbox,minimum height=0.40cm,minimum width=1.36cm,inner sep=2pt},
  schexit/.style={rounded corners=1.6pt,fill=schRecordFill,draw=schRecordLine,
    line width=0.35pt,inner sep=2.2pt,font=\schTiny,text=black!62,align=center},
}

\providecommand{\schbandtitle}[2]{%
  {\schSmall\bfseries #1}\\[0.4pt]{\schTiny\color{schMuted}#2}}

\providecommand{\schkey}[2]{%
  \tikz[baseline=-0.32ex]{\draw[rounded corners=0.5pt,line width=0.4pt,draw=#2,fill=#1]
    (0,0) rectangle (0.215,0.15);}}
\providecommand{\schlegend}[2]{%
  \node[anchor=east,font=\schTiny,text=schMuted,inner sep=0pt] at (#1,#2)
    {\schkey{schAgentFill}{schAgentLine}\,agent\hspace{0.30cm}%
     \schkey{white}{schLine}\,scripted\hspace{0.30cm}%
     \schkey{schHumanFill}{schHumanLine}\,researcher\hspace{0.30cm}%
     \schkey{schRecordFill}{schRecordLine}\,records};}

\providecommand{\schcard}[3]{\parbox[c][#1][t]{#2}{\raggedright #3}}
\providecommand{\schcardc}[3]{\parbox[c][#1][t]{#2}{\centering #3}}

\providecommand{\schcanvas}[1]{\path (0,0) rectangle (14.0,#1);}

